HackCar: a test platform for attacks and defenses on a cost-contained automotive architecture

In this paper, we introduce the design of HackCar, a testing platform for replicating attacks and defenses on a generic automotive system without requiring access to a complete vehicle. This platform empowers security researchers to illustrate the consequences of attacks targeting an automotive system on a realistic platform, facilitating the development and testing of security countermeasures against both existing and novel attacks. The HackCar platform is built upon an F1-10th model, to which various automotive-grade microcontrollers are connected through automotive communication protocols. This solution is crafted to be entirely modular, allowing for the creation of diverse test scenarios. Researchers and practitioners can thus develop innovative security solutions while adhering to the constraints of automotive-grade microcontrollers. We showcase our design by comparing it with a real, licensed, and unmodified vehicle. Additionally, we analyze the behavior of the HackCar in both an attack-free scenario and a scenario where an attack on in-vehicle communication is deployed.

==> sections/design.tex <==
\section{The HackCar test platform}
\label{s:implementation}
The design of the test platform starts with the definition of the operational scenarios that we want to support with the test platform.
In this work we focus on the definition of two simple operational scenarios that allows the demonstration of the consequences of cyber-attacks to the system and to test the applicability of already-published anomaly detectors for in-vehicle communication. We remark that we do not focus on discussing novel attack scenarios nor novel detection techniques, since this is beyond the scope of this work.
The two operational scenarios on which the design of the test platform is based are:
\begin{enumerate}
    \item \textbf{ManualAEB}, where the platform is manually controlled by an external controller and an Automatic Emergency Braking (AEB) system is enable to replicate a \emph{level 1} ADAS;
    \item \textbf{AutoDrive}, where the platform is able to move on a pre-defined route without requiring any external controller and with the AEB system enabled, replicating the functionality of a \emph{level 3+} ADAS.
\end{enumerate}

Hence, to support these two operational scenarios the requirements of the test platform (assuming that the actuators to replica the behavior of a vehicle by accelerating, steering and breaking are supported) can be summarized as follows:
\begin{itemize}
    \item wireless interface for the remote controller;
    \item sensing system for forward-object detection;
    \item on-board controller to operate on the braking system (for both scenarios) and the accelerating system (in the \emph{AutoDrive} scenario);
    \item on-board controller with the ability to switch between the two operational modes.
\end{itemize}

Moreover, as an additional requirement we include a dedicated microcontroller to support different attacks at in-vehicle network level. 

